RankRAG: Unifying Context Ranking with Retrieval-Augmented Generation in LLMs

Large language models (LLMs) typically utilize the top-k contexts from a retriever in retrieval-augmented generation (RAG). In this work, we propose a novel instruction fine-tuning framework RankRAG, which instruction-tunes a single LLM for the dual purpose of context ranking and answer generation in RAG. In particular, the instruction-tuned LLMs work surprisingly well by adding a small fraction of ranking data into the training blend, and outperform existing expert ranking models, including the same LLM exclusively fine-tuned on a large amount of ranking data. For generation, we compare our model with many strong baselines, including GPT-4-0613, GPT-4-turbo-2024-0409, and ChatQA-1.5, an open-sourced model with the state-of-the-art performance on RAG benchmarks. Specifically, our Llama3-RankRAG significantly outperforms Llama3-ChatQA-1.5 and GPT-4 models on nine knowledge-intensive benchmarks. In addition, it also performs comparably to GPT-4 on five RAG benchmarks in the biomedical domain without instruction fine-tuning on biomedical data, demonstrating its superb capability for generalization to new domains.

==> tables/human.tex <==
\begin{wraptable}{r}{0.55\linewidth}
\vspace{-3ex}
\renewcommand\arraystretch{0.9}
  \caption{Human evaluation (A/B testing) comparing \ours{} and ChatQA-1.5 on ConvQA datasets.\vspace{-1ex}}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccc}   \toprule
    %   \bfseries Dataset ($\rightarrow$) & \multicolumn{2}{c}{\bfseries E-SNLI} & \multicolumn{2}{c}{\bfseries OpenbookQA} & \bfseries StrategyQA  \\
    % \cmidrule(lr){2-3}   \cmidrule(lr){4-5}   \cmidrule(lr){6-6} 
   \bf Datasets &\bf Size &\bf \ours{} Win &\bf Tie &\bf ChatQA-1.5 Win  \\ \midrule
   \multirow{2}{*}{Doc2dial} & 8B & 23.5\% &	55.0\% &	21.5\%\\
    & 70B & 24.0\%	&55.0\% &	21.0\%\\
    \midrule
   \multirow{2}{*}{Inscit} & 8B &31.5\% &	42.0\% &	26.5\% \\
    & 70B & 36.0\% &	40.0\%	 &24.0\%\\
    \midrule
   \multirow{2}{*}{TopiOCQA} & 8B & 23.0\% & 56.5\% & 20.5\% \\
    & 70B & 26.0\% & 46.0\% & 28.0\% \\
    \bottomrule 
    \end{tabular}
}
    \label{tab:human_study}
\end{wraptable}
\vspace{-0.5ex}


==> tables/main_no_kilt.tex <==

\begin{table*}[t]\small
\centering
\renewcommand\arraystretch{0.95}
\caption{Results of \ours and baselines on 10 datasets.  
All results are under \emph{zero-shot} evaluation without additional demonstrations. 
Results unavailable in public reports are marked as ``--''.
}
\label{tab:main}
% \vspace{5pt}
% \setlength{\tabcolsep}{3.25pt}
\resizebox{1.00\linewidth}{!}{
\begin{tabular}{l|cccccccccc}
\toprule
\textbf{Task (Zero-Shot)} & \textbf{NQ} & \textbf{TriviaQA} & \textbf{PopQA} & \textbf{HotpotQA}  & \textbf{2WikimQA}  & \textbf{FEVER} & \textbf{MMLU} &  
% \textbf{WoW} &
\textbf{Doc2Dial} &	\textbf{TopiOCQA} &	\textbf{Inscit} \\
\midrule
\textbf{Metric} &  EM & EM / Acc. & EM / Acc. & EM / F1 & EM / F1 & Acc. & Acc. & F1 & F1 & F1 \\
\midrule
\multicolumn{6}{l}{\color{black}\textit{Without Retrieval-Augmented Generation}} \\
\midrule
% Fill in your data below this line
% GPT-3  175B~\cite{gpt3} & 14.6 & 64.3 \\ 
InstructGPT~(\citeauthor{ouyang2022training}) & 29.9 & 65.8 / 73.2 & -- / -- & 26.0 / 38.2 & 27.2 / 34.8 & 77.6 & 60.2 & -- & -- & --\\
% \midrule
% PaLM 540B  & \multirow{2}{*}{21.2} & \multirow{2}{*}{\textbf{76.9}} & \multirow{2}{*}{-} & \multirow{2}{*}{\textbf{80.8 / 75.5}} & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \multirow{2}{*}{\textbf{69.4}} \\
% (\citeauthor{chowdhery2022palm}) \\
PaLM2 540B~(\citeauthor{anil2023palm}) & 21.2 & 76.9 / -- & -- / --  & -- / -- & -- / -- & -- & 69.3 & -- & --  & -- \\
% Llama 65B   & \multirow{2}{*}{23.8} & \multirow{2}{*}{68.2} & \multirow{2}{*}{-} & \multirow{2}{*}{- / -} & \multirow{2}{*}{- / 79.4} & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \multirow{2}{*}{-} \\
% (\citeauthor{llama}) \\
% \midrule
% Llama 2 70B   & \multirow{2}{*}{25.3} & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \multirow{2}{*}{- / -} & \multirow{2}{*}{- / \textbf{80.7}} & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \multirow{2}{*}{-} \\
% (\citeauthor{llama2}) \\
% \midrule
% GLaM 64B \cite{du2021glam} & 37.5 & 71.3 \\
FLAN-LaMDA 137B~(\citeauthor{wei2021finetuned}) & 20.7 & 68.1 / -- & -- / --  & -- / -- & -- / -- & -- & -- / -- & --  & -- & --   \\
GPT-3.5~(\citeauthor{chatgpt}) & 35.1 & 70.1 / 81.3 & 28.4 / 32.2 & 29.9 / 42.0 & 23.9 / 30.4 & 82.7 & 70.0 & 20.1 &	28.5 &	27.2\\
GPT-4~(\citeauthor{gpt4}) & 37.2 & 72.6 / 85.1 & 31.3 / 34.8 & 34.5 / 46.9 & 29.8 / 36.6 & 87.7 & 75.5 & 27.6 &	30.1 &	27.0 \\

\midrule
\multicolumn{6}{l}{\color{black}\textit{With Retrieval-Augmented Generation}} \\
% Llama 2 RAG 70B \hfill & \multirow{2}{*}{37.7} & \multirow{2}{*}{65.6} & \multirow{2}{*}{53.4} & \multirow{2}{*}{71.4 / 64.1} & \multirow{2}{*}{73.4 / 66.2} & \multirow{2}{*}{69.7} & \multirow{2}{*}{52.7} & \multirow{2}{*}{57.2} \\ \midrule 
\midrule
% \multicolumn{6}{l}{\color{black}\textit{With Retrieval-Augmented Training}} \\
% \midrule
% Retro 7.5B \hfill & \multirow{2}{*}{8.9} & \multirow{2}{*}{36.0} & \multirow{2}{*}{-} & \multirow{2}{*}{- / -} & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \multirow{2}{*}{-} \\
% (\cite{borgeaud2022improving}) \\
% \midrule
% Retro++ 9B  \hfill & \multirow{2}{*}{25.8} & \multirow{2}{*}{48.3} & \multirow{2}{*}{-} & \multirow{2}{*}{- / -} & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \multirow{2}{*}{-} \\
% (\cite{wang2023shall}) \\
Atlas 11B (\citeauthor{atlas}) \hfill& 26.7 & 56.9 / -- & -- / -- & 34.7 / --&-- / --  & 77.0 & 45.7 
% & 15.0 
& -- & -- & -- \\ 
Raven  11B (\citeauthor{huang2023raven}) & {29.6} & {65.7} / -- & -- / -- & -- / -- & -- / -- & -- & 48.9 & --  & -- & --  \\
Self-RAG 7B~(\citeauthor{asai2024selfrag}) \hfill & -- & -- / 66.4 & -- / 54.9 & -- / -- & -- / -- & -- & -- & --  & -- &--  \\
Self-RAG 13B~(\citeauthor{asai2024selfrag})  &  -- & -- / 69.3 &  -- / 55.8 & -- / -- & -- / -- & -- & -- & -- & -- &-- \\
RECOMP 20B (\citeauthor{xu2024recomp}) & 37.0 & 59.0 / -- & -- / -- & 30.4 / 40.1 & -- / -- & --  & -- & --  & -- & -- \\
In-context RALM 33B (\citeauthor{ram2023context}) & 32.3 & 62.7 / -- & -- / -- & -- / -- & -- / -- & --  & -- & --  & -- & -- \\
InstructRetro 43B~(\citeauthor{wang2023instructretro}) \hfill &  38.9 & 65.6 / -- & -- & -- / -- & -- / -- & -- & -- & 36.0 & -- & --  \\
RA-DIT 65B~(\citeauthor{lin2024radit})  \hfill & 35.2 & 75.4 / -- & -- / -- & 39.7 / -- & -- / -- & 80.7 & 64.6 
% & 16.3 
& -- & -- & -- \\
Llama3-Instruct 8B~(\citeauthor{llama3}) & 31.6 & 57.1 / 74.6 &  34.9 / 55.8 & 19.9 / 35.8 & 9.6 / 25.2 & 88.9 & 51.5 & 33.6 & 44.9 & 32.6 \\
% Llama 3-Instruct 8B~\citep{llama3} & 31.61 & 57.10 / 74.60 &  34.88 / 59.83 & 19.86 / 35.76 & 9.57 / 25.20 & 88.93 & 51.46 
% % & 14.80 
% & 32.05 & 47.33 & 31.60 \\
Llama3-Instruct 70B~(\citeauthor{llama3}) & 37.2 & 67.6 / 79.6 & 45.3 / 56.4 & 25.5 / 43.3 & 13.5 / 27.9 & 91.4 & 70.7 & 37.9 & 49.7 & 36.2 \\
% Llama 3-Instruct 70B~\citep{llama3} & 37.25 & 67.65 / 79.65 & 45.32 / 59.67 & 25.54 / 43.27 & WIP & 91.39 & 70.77 
% % & 15.81 
% & 37.88 & 49.72 & 36.23 \\
Llama3-ChatQA-1.5 8B~(\citeauthor{liu2024chatqa}) \hfill  & 44.1 & 64.3 / 75.2 & 52.6 / 59.8 & 33.4 / 44.6& 26.8 / 31.9 & 90.9 & 55.7 &  39.3 & 49.9 & 30.1 \\
% 33.4/44.6
% 42.2/54.4
% ChatQA-1.5 8B~\cite{liu2024chatqa} \hfill  & 44.05 & 64.33 / 75.26 & 50.68 / 62.12 & 31.56 / 42.13 & 26.81 / 31.93 & 90.88 & 55.76 
% % & 15.87 
% &  39.33 & 49.96 & 30.10 \\
Llama3-ChatQA-1.5 70B~(\citeauthor{liu2024chatqa}) \hfill  & 46.2 & 68.9 / 80.4 & 50.9 / 58.3 & 42.2 / 54.4 & 34.9 / 37.4 & 92.7 & 71.3 
& 41.3 & 55.6 & 32.3 \\
% ChatQA-1.5 70B~\cite{liu2024chatqa} \hfill  & 46.20 & 68.95 / 80.44 & 48.89 / 61.33 & 35.89 / 47.27 & 34.94 / 37.41 & 92.70 & 71.29 
% & 16.07 
% & 41.26 & 55.63 & 32.31 \\
\midrule
\rowcolor{green!12} Llama3-\ours 8B & 46.1 & 68.8 / 79.9 & 57.6 / 64.1  & 35.3 / 46.7 & 31.4 / 36.9 & 92.0 & 60.3 
& 40.4 & 50.4 & 33.3  \\ 
% \rowcolor{green!15} \ours 8B & 46.09 & 68.81 / 79.89 & 57.61 / 67.55  & 35.29 / 46.74 & 31.36 / 36.88 & 91.99 & 60.33 
% & 16.20 
% & 40.36 & 50.43 & 33.31  \\ 
\rowcolor{green!12} Llama3-\ours 70B & \textbf{50.0} & \textbf{72.6} / \textbf{82.9} & \textbf{59.9} / \textbf{65.4} & \textbf{42.7} / \textbf{55.4} & \textbf{38.2} / \textbf{43.9} & \textbf{93.8} &  \textbf{73.7} & 41.5 & 52.8 & 35.2  \\ 
% \rowcolor{green!15} \ours 70B & \textbf{50.00} & \textbf{72.62} / \textbf{82.89} & \textbf{59.90} / \textbf{68.98} & \textbf{42.70} / \textbf{55.36} & \textbf{38.17} / \textbf{43.90} & \textbf{93.81} &  \textbf{73.71} 
% & 16.25 
% & 41.48 & 52.81 & 35.23  \\ 

% InstructRetro 43B \hfill  & \textbf{38.9} & 65.6 & \textbf{57.4} & \textbf{75.6} / \textbf{69.3} & 77.1 / 70.4 & \textbf{76.2} & \textbf{60.0} & {54.8} \\
% \tiny{(w/o encoder, Avg: +7\%)} & \tiny{(+5.14\%)} & \tiny{(+0.92\%)} & \tiny{(+9.54\%)} & \tiny{(+6.93\%)} & \tiny{(+6.49\%)} & \tiny{(+6.57\%)} & \tiny{(+11.32\%)} & \tiny{(+5.79\%)} \\
% InstructRetro 48B \hfill  &  38.6 & 65.4 &  57.0 & 74.8 / 67.7 & 76.4 / 69.0 & 76.1 & 59.8 & 54.6 \\
% \tiny{(w/ encoder, Avg: +6\%)} & \tiny{(+4.32\%)} & \tiny{(+0.62\%)} & \tiny{(+8.78\%)} & \tiny{(+5.80\%)} & \tiny{(+5.52\%)} & \tiny{(+6.43\%)} & \tiny{(+10.95\%)} & \tiny{(+5.41\%)} \\
\midrule
\multicolumn{10}{l}{\textbf{For reference}: \emph{Using InstructGPT or CodeX ($\sim$175B)~\citep{ouyang2022training} as the Backbone LLM. Most of the results are from~\citep{refeed}.}} \\
\midrule 
GenRead~(\citeauthor{genread}) & 32.5 & 66.2 / -- & 46.0 / -- & 26.0 / 38.2 & -- & 80.4 & -- & -- & -- &  -- \\ % (Yu et al. 2023a)
Self-Prompting~(\citeauthor{self_prompting})  & 36.2 & 66.8 / -- & -- / -- & -- / -- & -- & -- & -- & -- & -- & --  \\ %(Li et al. 2024)
Retrieve-Read~(\citeauthor{lazaridou2022internet}) & 31.7 & 61.4 / -- & -- / -- & 35.2 / 38.0 & 27.7 / -- & 82.7 & -- & -- & -- & -- \\%(lazaridou et al.)
RePlug~(\citeauthor{shi2023replug}) & 34.7 & 66.5 / -- & -- / -- & 37.5 / 41.2 &  -- / -- & -- & 71.8 & -- & -- & --   \\ %(Shi et al., 2024)
ReFeed~(\citeauthor{refeed}) & 39.6 & 68.9 / -- & -- / -- & 41.5 / 45.1 & -- / -- & -- & -- & -- &  -- & -- \\ %(Yu et al., 2023b)
\bottomrule
\end{tabular}
}
\end{table*}

